On the Validity of Modeling SGD with Stochastic Differential Equations (SDEs)

It is generally recognized that finite learning rate (LR), in contrast to infinitesimal LR, is important for good generalization in real-life deep nets. Most attempted explanations propose approximating finite-LR SGD with Ito Stochastic Differential Equations (SDEs), but formal justification for this approximation (e.g., (Li et al., 2019)) only applies to SGD with tiny LR. Experimental verification of the approximation appears computationally infeasible. The current paper clarifies the picture with the following contributions: (a) An efficient simulation algorithm SVAG that provably converges to the conventionally used Ito SDE approximation. (b) A theoretically motivated testable necessary condition for the SDE approximation and its most famous implication, the linear scaling rule (Goyal et al., 2017), to hold. (c) Experiments using this simulation to demonstrate that the previously proposed SDE approximation can meaningfully capture the training and generalization properties of common deep nets.

==> checklist.tex <==
\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} We describe the restrictions that the assumptions place on the applicability of our theory when relevant.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} We discuss how our necessary condition for LSR can aid practitioners in making their hyperparameter search more efficient. We also note in the paper that as $l$ in SVAG increases, it takes longer for each experiment to run, thereby consuming more resources.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} We discuss the assumptions required for \Cref{thm:sde_svag} in a remark below the theorem statement. We furthermore state and discuss the equilibrium assumptions needed in \Cref{sec:failure_mode_1}.
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} We include a proof overview for SVAG in \Cref{sec:svag} and defer all of the formal proofs to the appendix. \Cref{appsec:svag_details} has the full SVAG proof, and \Cref{appsec:omit_proofs_lsr} has detailed proofs for the results in \Cref{sec:failure_mode_1}. 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} We will upload a zip file with the anonymized code.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We cite the tools in \Cref{sec:app_exp}.
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} We built a codebase from some existing code to run experiments and will upload it.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{} We use standard open-access datasets: CIFAR-10, CIFAR-100, and Street View House Numbers (SVHN).
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
     \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> experiments.tex <==

\section{Experiments and Discussion}\label{sec:lsr_verify}\label{sec:svag_verify}

\subsection{Figures}
We can move this to wherever needed, just some placeholder figures.

e rest is 


\iffalse
\subsection{Verifying the LSI Condition}
We empirically test if the necessary condition proposed in \Cref{thm:lsr_condition} accurately captures when the LSR works using a PreResNet-32 \cite{he2016identity} modified to be scale-invariant. In particular, as the batch size increases, the gradient noise $N_t$ decreases, so we expect LSR to fail for large batch sizes. We observe this to be true in \Cref{fig:lsr_acc_gnr}.


\begin{figure}
\centering
\begin{subfigure}
  \centering
  \centerline{\includegraphics[width=0.5\textwidth]{img/Acc_LSR.png}}
  \caption{Accuracy}
\end{subfigure}%
\begin{subfigure}
  \centering
  \centerline{\includegraphics[width=\linewidth]{img/GNR_LSR.png}}
  \caption{$\max(G_t/N_t)$}
\end{subfigure}
\caption{We train a scale-invariant PreResNet-32 with different batch sizes, scaling the learning rate as prescribed by the linear scaling rule (\Cref{def:lsr}). The degradation of accuracy for large batch sizes corresponds to an increase in $\max(G_t/N_t)$, providing evidence that \Cref{thm:lsr_condition} is meaningful in practice.}
\label{fig:lsr_acc_gnr}
\end{figure}


\subsection{Verifying SVAG Approximation Theorems}
If the train/test curve of the deep nets remain almost the same when training with SVAG with increasing $l$, then it suggests that SDE is a good approximation for SGD and it makes sense to study the implicit bias of SGD via SDE. In \Cref{fig:acc_vs_k}, we train a PreResNet-32 with SVAG parametrized by $l=2^i$ for $i\in\{1,2,\ldots,7\}$, and confirmed that the train/test curves do highly overlap for different $l$. Also we note the SVAG ($l>1$) has smaller oscillation than SGD ($l=1$) before the first LR decay (at epoch $80$), but in the latter phase, the curves are match similar.

%We experimentally check that the SVAG algorithm in \Cref{sec:svag} is a good approximation: one step of training in the baseline algorithm should correspond to $l$ steps of training with SVAG with parameter $l$. We observe this to be true in \Cref{fig:acc_vs_k}. 

\begin{figure}
\centering
\begin{subfigure}
  \centering
  \centerline{\includegraphics[width=\linewidth]{img/trainaccvsk.png}}
  \caption{Train Accuracy (smoothed)}
  \label{fig:train_vs_k}
\end{subfigure}%
\begin{subfigure}
  \centering
\centerline{\includegraphics[width=\linewidth]{img/valaccvsk.png}}
  \caption{Validation Accuracy}
  \label{fig:val_vs_k}
\end{subfigure}
\caption{Training and validation accuracy curves for different $l$ values using SVAG. The $x$ axis has ``effective steps'' $= lt$, where $t$ is the number of steps of gradient descent. Per \Cref{thm:sde_svag}, we expect all of these trajectories to be the same.}
\label{fig:acc_vs_k}
\end{figure}

\paragraph{Discussion}
We observe that accuracy can degrade slightly for small batch sizes as well (\Cref{fig:lsr_acc_gnr}). We hypothesize that this is because PreResNet-32 uses batch normalization, and the batch statistics cannot be computed as accurately from smaller batches. To verify our hypothesis, we need to train the model with other normalization schemes, such as group normalization or layer normalization. 
\fi

==> lsi.tex <==
\subsection{Linear Scaling Rule and Linear Scaling Invariance}\label{sec:warmup}
%Before diving into our main result, we will first talk about the probably most important and well-known consequence of the SDE approximation, which is that if it holds, then the Linear Scaling Invariance defined below also holds.
In this section, we show the common intuition that if the SDE approximation holds, then the linear scaling rule (~\Cref{def:lsr}) will not affect model performance.
However, the SDE approximation provides an incomplete justification for the linear scaling rule, because the rule can work even if the approximation does not hold.

\cite{goyal2017accurate} originally justify LSR by suggesting that $\kappa$ consecutive $\eta$-sized steps with batch size $B$ can sometimes be approximated with a single $\kappa\eta$-sized step with batch size $\kappa B$.
Hence, LSR holds when there is low discretization error.

Since LSR only modifies the batch size and learning rate, we assume an arbitrary but fixed training setting (i.e., model architecture, dataset, and random seed) and baseline choice of $B$ and $\eta$ for the below definitions.
%We note that there are two interpretations of the rule, which we expand below.
\begin{definition}[$\kappa$-LSR Model]
	A model trained using batch size $\kappa B$ and learning rate $\kappa\eta$.
\end{definition}

\begin{definition}[Weak Linear Scaling Invariance]
	A training setting and a given $\kappa$ exhibit weak linear scaling invariance (or weak LSI) if the baseline and $\kappa$-LSR models have the same final performance on a held-out dataset.
\end{definition}
Note that even in a fixed training setting, LSI may hold only for certain $\kappa$ values, as was first observed in \cite{goyal2017accurate}.
Weak LSI implies that applying LSR with a specified $\kappa$ preserves the generalization properties of the trained model.
Weak LSI is difficult to study in terms of the SDE approximation, because models with different training trajectories can have the same generalization properties.
Hence, we define a stronger sense of LSI below.
\begin{definition}[Weight Norm]
	For a model trained with batch size $B$ and learning rate $\eta$, we define $R_\infty^{B, \eta} := \lim_{T\to\infty} \E\frac{1}{T} \sum_t \|x_t\|^2 = \lim_{T\to\infty} \E \|x_t\|^2$.
\end{definition}
\begin{definition}[Gradient Norm]
	For a model trained with batch size $B$ and learning rate $\eta$, we define $G_\infty^{B, \eta} := \lim_{T\to\infty} \E\frac{1}{T} \sum_t \|\nabla \Loss(x_t)\|^2 = \lim_{T\to\infty} \E \|\nabla \Loss(x_t)\|^2$.
\end{definition}
\begin{definition}[Gradient Noise]
	For a model trained with batch size $B$ and learning rate $\eta$, we define $N_\infty^{B, \eta} := \lim_{T\to\infty} \E\frac{1}{T} \sum_t \Tr(\Sigma(x_{t}))= \lim_{T\to\infty} \E \Tr(\Sigma(x_{t})) $.
\end{definition}
Under LSR, the learning rate $\eta$ is prescribed by the choice of batch size $B$, so we shorten the notation to $R_\infty^B$, $G_\infty^B$, and $N_\infty^B$, respectively.
When we are discussing these quantities for any SGD setting, we shorten them to $R_\infty$, $G_\infty$, and $N_\infty$, respectively.
\begin{definition}[$C$-Strong Linear Scaling Invariance]\label{def:lsi}
	A training setting and a given $\kappa$ exhibit $C$-strong LSI if, for a constant $0 < C < \sqrt{\kappa}$,  
\[\frac{1}{C}\le \frac{R^{B}_\infty}{R^{\kappa B}_\infty},\frac{N^{B}_\infty}{\kappa N^{\kappa B}_\infty},\frac{G^{B}_\infty}{G^{\kappa B}_\infty}\le C.\] 
\end{definition}
This definition informally states that the weight norm, gradient norm, and gradient noise of the baseline and $\kappa$-LSR models should be close to each other at equilibrium for strong LSI to hold.
Therefore, strong LSI implies weak LSI.
%Note that $N_\infty^{\kappa B} = \frac{1}{\kappa}N_\infty^B$.
%\zhiyuan{add definition of $R_{\infty}$, define $R_{\infty}^{B,\eta}$, and in the later theorem we will simply denote it by $R_{\infty}^{B}$ under the LSR.}

==> lsi_analysis.tex <==
\subsection{SDE Approximation Exhibits Strong LSI for Any $\kappa$}
We use $\Sigma^B(X)$ to denote the covariance of the gradient when the batch size is $B$, and therefore $\Sigma^B(X) = \frac{\Sigma^1(X)}{B}$.\footnote{Here we assume there's no BatchNorm is used in the network and thus the batch loss is the average of the individual losses.} 
Thus under LSR, $\eta\Sigma^B(X) = \frac{\eta}{B} \Sigma^1(X)$ is a constant independent of individual values of $\eta$ and $B$. 
Using~\Cref{eq:motivating_sde}, we can conclude that the SDE approximation exhibits strong LSI for all values of $\kappa$.

Hence, for a given training setting, if the SDE approximation accurately models the SGD dynamics, then the setting exhibits strong LSI for all values of $\kappa$.
As such, \cite{smith2020generalization} use the SDE approximation as an explanation for observing LSI in real-world training settings.
However, below, we demonstrate that a training setting can exhibit strong LSI even if the SDE approximation does not hold.
%For this reason, some existing work tries to argue that SGD dynamics exhibit LSI using the SDE approximation~\citep{smith2020generalization}. 

\subsection{Strong LSI Does Not Imply SDE Approximation Holds}\label{sec:sde_to_lsi}
Strong LSI can hold even when the SDE approximation fails, as we demonstrate through an example.
In particular, the SDE approximation requires a Gaussian noise distribution, and we show that LSI can hold for other noise distributions.\footnote{Here we used the Poisson process and indeed any Levy process would work.}

\begin{example}
Let $\N^+$ be the domain and each point $x\in\R$ is sampled from $\mu_\lambda$, where $\mu_\lambda$ is Poisson distribution with parameter $\lambda$, i.e. $\mu_\lambda(a) = \frac{\lambda^a e^{-\lambda}}{a!}$, $\forall a\in \N$. 
Consider a linear loss function, i.e., $\Loss_a(x) = ax$. 
For batch $\vB = \{a_i\}_{i=1}^B$, we define $\Loss_\vB(x) = \frac{\sum_{i=1}^B a_i}{B}x$. Therefore $B\nabla \Loss_\vB(x) \sim \mu_{B\lambda}$.

%Note that the convolution of two Poisson distributions with parameter $\lambda_1,\lambda_2$ is a Poisson distribution with parameter $\lambda_1+\lambda_2$. 
Starting from $x_0$, with learning rate $\eta$, batch size $B$, we have for all $k\in \left[1, \frac{N}{B}\right]$, 
\[ x_k = x_{k-1} - \eta \nabla\Loss_{\vB_k}(x_{k-1})\quad \Longrightarrow\quad -\frac{\eta}{B}x_{\frac{N}{B}} \sim\mu_{N\lambda}. \]

The implication follows from the fact that the convolution of two Poisson distributions with parameter $\lambda_1,\lambda_2$ is a Poisson distribution with parameter $\lambda_1+\lambda_2$. 
Therefore, as long as the $\frac{\eta}{B}$ is fixed, the resulting distribution of $x_{\frac{N}{B}}$ is independent of individual value of $B$ or $\eta$, which implies that strong LSI holds.
However, the distribution is Poisson but not Gaussian, thus is not close to the SDE,~\Cref{eq:motivating_sde}.  
\zhiyuan{What does the next sentence mean?}
Also this is an example where moving towards each side of LSR doesn't make the dynamics closer to the SDE,~\Cref{eq:motivating_sde}.%\footnote{Here we used the Poisson process and indeed any Levy process would work.}
\end{example}

 The above example shows that tiny learning rate plus  matched the first and second moments is not sufficient for SGD,~\Cref{eq:sgd_iter}, to be close to SDE,~\Cref{eq:motivating_sde}. As we will see from the proof later(e.g.\Cref{lem:D}), it also requires the third order moment to vanish.

In the next section, we describe a necessary but not sufficient condition for strong LSI to hold.

\subsection{Necessary Condition for Strong Linear Scaling Invariance}\label{sec:sgd_analysis}
\zhiyuan{What does this paragraph mean?}
In practice, \cite{li2020reconciling} observed that the dynamics of SGD tend to converge to a certain limiting distribution, due to the scale invariance induced by normalization layers in the network. 
While our approximation results only hold for finite time, below we will present a necessary condition for strong LSI (\Cref{def:lsi}).
 
Below we assume loss $\Loss_\vB$ is scale invariant for any $\Loss_{\vB}$, i.e., $\Loss_\vB(cx) = \Loss_\vB(x)$ for any $c>0$, where $\vB$ is the batch of data. 
We further assume $x_t$ converges in distribution, and thus the previously defined defined $R_\infty$, $N_\infty$, and $G_\infty$ exist.

\begin{definition}[Distance between SGD Iterates]
	We define $D_\infty := \lim_{T\to\infty} \E\frac{1}{T} \sum_t \|x_{t+1} - x_t\|^2$.
\end{definition}
The existence of $D_\infty$ is given by \Cref{lem:D_to_N_G}.        

\begin{lemma}[Existence of $D_\infty$]\label{lem:D_to_N_G}
	$ \E \|x_{t+1} - x_t\|^2 = \eta^2\left(\E\Tr(\Sigma(x_{t})) + \E\norm{\nabla \gL(x_t)}^2\right)$
\end{lemma}
In fact, we can relate $R_\infty$, $G_\infty$, and $N_\infty$ as follows.
\begin{lemma}\label{lem:R_to_G_N}
	$(1-\eta\lambda)R_\infty = \frac{\eta}{2\lambda}(G_\infty + N_\infty)$.

%	$D_\infty = \lim_{T\to\infty} \frac{1}{T} \sum_t \|x_{t+1} - x_t\|^2$. Under the 1st order SDE formulation,
%	\begin{equation*}
%		D_\infty = \eta^2 \lim_{T\to \infty} \frac{1}{T}\sum_{t=1}^T \left(\E\Tr(\Sigma(x_{t})) + \E\norm{\nabla \gL(x_t)}^2\right)
%	\end{equation*}
\end{lemma}

\begin{proof}
	By Theorem B.2 in \cite{li2020exp}, $R_\infty = \frac{D_\infty}{2\lambda \eta}$.  
	The proof is completed by applying \Cref{lem:D_to_N_G}.
	\zhiyuan{Need to adjust the proof for weight decay term?}
\end{proof}

We are interested in studying these quantities when training with different batch sizes and learning rates. Hence we denote $R^B_\infty$, $G^B_\infty$ and $N^B_\infty$ as the limits when the batch size is $B$ and the learning rate is $\eta$. 
\begin{theorem}\label{thm:lsr_condition}
For any $\kappa$ such that strong LSI holds, $ N^{\kappa B}_\infty\ge (\frac{1}{C^2} -\frac{1}{\kappa})G^{\kappa B}_\infty$.
\end{theorem}

\begin{remark}
    This theorem is a formal statement of the necessary condition for strong LSI to hold: $N_\infty^{\kappa B}$ must be larger than $G_\infty^{\kappa B}$. 
    We verify this experimentally in \Cref{sec:lsr_verify}.
    Because strong LSI implies that the SDE approximation holds, we can also interpret this theorem as a necessary condition for the SDE in \Cref{eq:motivating_sde} to correctly approximate SGD dynamics.
\end{remark}

\zhiyuan{Explanation of 2nd order SDE intuition}

\iffalse
\subsection{2nd Order SDE Approximation Accurately Models when LSI Holds}
We note that the commonly used 1st order SDE approximation shown in \Cref{eq:motivating_sde} does not predict that strong LSI will not hold in large batch size (i.e., low-noise) regimes.
However, the 2nd order SDE approximation does accurately model the necessary condition derived in \Cref{thm:lsr_condition}.
This is of interest to theoreticians who may now want to study the 2nd order approximation.

\sadhika{Proofs here - 1st order SDE misses $\|\nabla\Loss\|^2$ term and 2nd order SDE has it}
\fi



==> lsi_experiments.tex <==
%\subsection{Experimental Evidence for~\Cref{thm:lsi_GN}}
\iffalse 
\subsection{Experimental Evidence}\label{sec:lsr_verify}
We verify our theory for predicting the failure of Linear Scaling Rule using PreResNet-32 and VGG19 trained on CIFAR-10 (\Cref{fig:lsr_acc_gnr}). 
Our theory only asserts the failure of closeness of the equilibrium distributions regarding test functions $\Ri^{B},\Gi^B,\Ni^B$, but we observe that the final performances also differ when these test functions are apart from each other.
In particular, we note that the proposed necessary condition for failure of LSR (\Cref{def:lsr}), denoted by a red dashed line, is very close to the true failure of LSR.
Furthermore, although our theory only holds for scale-invariant nets, we found it to be meaningful even when most but not all parameters are scale-invariant (\Cref{sec:app_exp}).
\fi


%\subsection{Predicting the failure of Linear Scaling Invariance}

==> non_gaussian_noise.tex <==
\section{Failure of SDE Approximation Caused by Non-Gaussian noise}

\subsection{LSR can hold when SDE approximation breaks}\label{sec:counterexample}
%\subsection{LSR holds for any step size}
\begin{example}
Let $Z(t)$ be a $1$-dimensional Poisson process (Definition ??), where $Z(t)$ follows Poisson distribution with parameter $t$. 
We assume the distribution of the gradient on single sampled data $\gamma$, $\nabla L_\gamma(x)$ is the same as $Z(1)$ for any parameter $x$. 
For a batch $\vB$ of size B (with replacement), since Poisson process has independent increments, $\nabla \Loss_\vB(x):=\frac{1}{B}\sum_{\gamma \in \vB}\nabla \Loss_\gamma(x) \overset{d}{=} \frac{Z(B)}{B}$.

Thus for any constant $T$ and initialization $x_0 = 0$, performing SGD starting from $x_0$ for $\frac{T}{B}$ steps with LR $B\eta$ and batch size $B$, the distribution of $x_{\frac{T}{B}}$ is independent of $B$, i.e., 
\begin{align*} 
x_k = x_{k-1} - B\eta \nabla\Loss_{\vB_k}(x_{k-1}) \Longrightarrow 
x_{\frac{T}{B}} \overset{d}{=}  -\eta(\underbrace{Z(B)+Z(B)+\cdots+Z(B))}_{\frac{T}{B}\text{'s }Z(B)}\overset{d}{=}-\eta Z(T). 	
\end{align*}
\end{example}

Thus LSR holds for all batch size $B$. Below we consider the corresponding NGD~\eqref{eq:noisy_gd}, $\{\hat{x}_k\}$, where

\begin{align*}
\hat{x}_k =& \hat{x}_{k-1}-B\eta \E\nabla \Loss_{\vB_k}(\hat{x}_{k-1})+ B\eta \sqrt{\E(\nabla \Loss_{\vB_k}-\E\nabla \Loss_{\vB_k})^2}z_{k-1}	\\
= & \hat{x}_{k-1} - B\eta \E\frac{Z(B)}{B} + B\eta \sqrt{\E(\frac{Z(B)}{B}-\E \frac{Z(B)}{B})^2}z_{k-1}z_{k-1}\\
=& \hat{x}_{k-1} - B\eta + \eta \sqrt{B\E(Z(1)-\E Z(1))^2}z_{k-1}\\
=& \hat{x}_{k-1} - B\eta + \eta\sqrt{B} z_{k-1},
\end{align*}
and $\{z_i\}_{i=0}^{\frac{T}{B}-1}\overset{i.i.d.}{\sim}N(0,1)$.

Thus it holds that $\hat{x}_{\frac{T}{B}} = -\eta T + \eta \sum_{k=0}^{\frac{T}{B}-1} z_{k-1} \overset{d}{=} -\eta (T + W_T)$, where $W_T$ is a Wiener process, meaning the NGD final iterate is also independent of $B$, and constant away form  the final iterate $x_{\frac{T}{B}}\overset{d}{=} -\eta Z(T)$. Indeed we can show the same result for Ito SDE~\eqref{eq:motivating_sde}, $\dd X_t = - \dd t + \sqrt{\eta} \dd W_t$: \[X_{\frac{T}{B}\cdot B\eta } = X_{\eta T} = \int_{t=0}^{\eta T} (-\dd t+\sqrt{\eta} \dd W_t) =-\eta T + \sqrt{\eta }W_{\eta T} \overset{d}{=} -\eta T + \eta W_T.\]

Thus we conclude that \textbf{LSR holds but SDE approximation fails}. Since NGD achieves the same distribution as Ito SDE, \textbf{the gap is solely caused by non-gaussian noise}.

==> sde_failure_lsr.tex <==
\newcommand{\bR}{\overline{R}}
\newcommand{\bG}{\overline{G}}
\newcommand{\bN}{\overline{N}}

\newcommand{\Ri}{R_\infty}
\newcommand{\Gi}{G_\infty}
\newcommand{\Ni}{N_\infty}

\newcommand{\bRi}{\bR_\infty}
\newcommand{\bGi}{\bG_\infty}
\newcommand{\bNi}{\bN_\infty}


\section{Provable Failure of SDE Approximation and LSR by Discretization Error}\label{sec:failure_mode_1}

In this section, we show how discretization error, or large LR, leads to a provable failure of SDE approximation and LSR for scale invariant networks at equilibrium (i.e., nets equipped with BatchNorm~\cite{ioffe2015batch} and GroupNorm~\cite{wu2018group}). When trained with constant LR and Weight Decay (WD), \cite{li2020reconciling} shows that the parameter norm will converge and finds experimentally that the training loss will reach some plateau, suggesting the existence of equilibrium. Below we assume the existence of such equilibrium for both SGD/SDE and will show if LR $\eta\gtrsim \frac{\bNi }{\bGi}$, which is the \emph{Noise-Signal-Ratio} (NSR) of SDE at equilibrium (see \Cref{def:lsi}). Since this condition doesn't involve the shape of noise and thus holds even for gaussian noise, the failure is solely caused by discretization error.
 
%The network will  when the LR $\eta$ is larger than the \emph{Noise-signal-ratio} of SGD/SDE at equilibrium. 
%In this section, we provide a sufficient condition on LR to answer the following question for normalized networks (e.g. BatchNorm~\cite{ioffe2015batch} and GroupNorm~\cite{wu2018group}) trained by SGD + Weight Decay (WD):
%\emph{Given a fixed SDE~\eqref{eq:sde_wd}, when does SGD~\eqref{eq:sgd_wd} with matching moments have a very different equilibrium?}

We consider the following SDE~\eqref{eq:sde_wd} and the moment-matching SGD~\eqref{eq:sgd_wd} satisfying $\Loss(x) = \E\Loss_\gamma(x)$ and $\overline{\Sigma}(x) = \eta\Sigma(x)$ where $ \Sigma(x)$ is the covariance of $\nabla \Loss_\gamma(x)$. We assume for all $\gamma$, $\Loss_\gamma$ is \emph{scale invariant}~\cite{arora2018theoretical,Li2020An}, i.e., $\Loss_\gamma(x) = \Loss_\gamma(cx)$,  $\forall c>0$ and $x\in\R^d/\{0\}$, which implies $\inp{\nabla \Loss_\gamma(x)}{x} = 0$.
\begin{align}
\!\!\!\!\dd X_t\! =&\! - \nabla \big(\Loss(X_t) + \frac{\lambda}{2} |X_t|^2\big) \dd t +  {\overline{\Sigma}^{1/2}(X_t)} \dd W_t \label{eq:sde_wd}\\
x_{k+1} =& x_k - \eta \nabla \big(\Loss_{\gamma_k}(x_k) + \frac{\lambda}{2} |x_k|^2\big)  \label{eq:sgd_wd}
\end{align}

We will measure the closeness of two distributions by three test functions: squared weight norm $|x|^2$, squared gradient norm $|\nabla\Loss(x)|^2$ and trace of noise covariance, $\Tr[\Sigma(x)]$. 
We say two equilibriums are different, if at least one of these test functions differ by a multiplicative constant.


\begin{definition}[$C$-closeness]\label{def:lsi}
Assuming the existence of the following limits, we use \\
 $R_\infty:= \lim\limits_{t\to \infty} E|x_t|^2$, \hspace{1.40cm}$\bR_\infty:= \lim\limits_{t\to \infty} E|X_t|^2$,\\
 $G_\infty:= \lim\limits_{t\to \infty}\E |\nabla \Loss(x_t)|^2$,\hspace{0.78cm}$\bG_\infty:= \lim\limits_{t\to \infty}\E |\nabla \Loss(X_t)|^2$,\\
 $N_\infty:= \lim\limits_{t\to \infty} \E[\Tr[\Sigma(x_t)]$, \hspace{0.46cm}$\bN_\infty:= \lim\limits_{t\to \infty} \E[\Tr[\overline{\Sigma}(X_t)]$ \\
to denote the limiting squared norm, gradient norm and trace of covariance for SGD~\eqref{eq:sgd_wd} and   SDE~\eqref{eq:sde_wd}.  
We say the two equilibriums are \emph{$C$-close} to each other iff 
\begin{align}\label{eq:C_close}
	\frac{1}{C}\le \frac{R_\infty}{\bR_\infty},\frac{G_\infty}{\bG_\infty},\frac{ \eta N_\infty}{\bN_\infty}\le C.
\end{align}
\end{definition}
Now we will show formally how the above defined $C$-closeness will break for large LR. 
%Formally we have the theorem below:

\begin{theorem}\label{thm:eq_sde_sgd}
The equilibriums of~\eqref{eq:sgd_wd} and \eqref{eq:sde_wd} are $C$-close $\Longrightarrow$ 
	$\eta \le \frac{\bNi}{\bGi}(C^2-1)$ and $\frac{1}{C^2-1}\le \frac{\Ni}{\Gi}$.
\end{theorem}

\begin{figure*}[t]
    \centering\vspace{-0.3cm}
    \includegraphics[width=\textwidth]{img/multiplot_CIFAR10.pdf}
    \vspace{-0.7cm}
    \caption{ 
%We train PreResNet-32 with BatchNorm (BN, left) and GroupNorm (GN, middle) as well as VGG19 with GN (right) on CIFAR-10 with batch sizes $B=2^i$ for $i\in[1,11]$ using LSR (\Cref{def:lsr}).
Experimental verification for our theory on predicting the failure of Linear Scaling Rule. 
We modify PreResNet-32 and VGG-19 to be scale-invariant (According to Appendix C of \cite{li2020reconciling}).
All three settings use the same lr schedule, LR$=0.8$ initially and is decayed by $0.1$ at epoch $250$ with $300$ epochs total budget.  Here, $G_t$ and $N_t$ are the empirical estimations of $\Gi$ and $\Ni$ taken after reaching equilibrium in the first phase (before LR decay).
%    We report $G_t/N_t$ (top) at equilibrium during the 1st phase of training as well as the final train, final test, and 1st phase equilibrium train accuracies (bottom).
    %Per the approximated version of \Cref{thm:lsr_kappa_bound}, i.e., $B^*=\kappa B \lesssim C^2B{\Ni^B}/{\Gi^B}$, we report the maximal and minimal predicted critical batch size using baseline runs of different batch sizes $B$, which are the intersections between the black horizontal line ($\nicefrac{G_t}{N_t}=C^2$) and the green (blue) lines respectively.
     Per the approximated version of \Cref{thm:lsr_kappa_bound}, i.e., $B^*=\kappa B \lesssim C^2B{\Ni^B}/{\Gi^B}$, we use baseline runs with different batch sizes $B$ to report the maximal and minimal predicted critical batch size, defined as the intersection of the threshold ($\nicefrac{G_t}{N_t}=C^2$) with the green and blue lines, respectively.
%    and use this approximation to predict the smallest batch size (marked by a red dashed line) where the necessary condition for LSR will be violated (i.e., $G_t/N_t$ surpasses $C^2$, denoted by a black horizontal line). 
    We choose a threshold of $C^2 = 2$, and consider LSR to fail if the final test error exceeds the lowest achieved test error by more than 20\% of its value, marked by the red region on the plot. Surprisingly, it turns out the condition in \Cref{thm:lsr_kappa_bound} is not only necessary, but also close to sufficient. 
    Further settings and discussion is in \Cref{sec:app_exp}. 
    }\vspace{-0.cm}
    \label{fig:lsr_acc_gnr}\label{sec:lsr_verify}
\end{figure*}

\begin{proof}[Proof of \Cref{thm:eq_sde_sgd}]

Following the derivation in \citep{li2020reconciling}, we have 
\begin{align}\label{eq:norm_sde_wd}
\frac{\dd}{\dd t}\E|X_t|^2 = -2\lambda\E |X_t|^2 + \E\Tr[\Sigma(X_t)].	
\end{align}
It can be shown that for SGD~\eqref{eq:sgd_wd}, it holds that
\begin{equation}\label{eq:norm_sgd_wd}	
\begin{split}
	\E|x_{k+1}|^2 -\E |x_{k}|^2=& (1-\eta\lambda)^2\E |x_{k}|^2 + \eta^2\E|\nabla \Loss_{\gamma_k}(x_k)|^2 -\E |x_{k}|^2\\
	\!\!\!\!\!\!= & \eta\lambda(-2\!+\!\eta\lambda)\E |x_{k}|^2\! +\! \eta^2\E |\nabla\Loss(x_k)|^2 +\eta^2\E \Tr[\Sigma(x_k)]
\end{split}
\end{equation}
If both $x_k$ and $X_t$ have reached their equilibriums, both LHS of \eqref{eq:norm_sde_wd} and \eqref{eq:norm_sgd_wd} are $0$, and therefore 
\begin{align}
	(2-\eta\lambda)\lambda\Ri &= \eta \Gi + \eta\Ni, \label{eq:RGN_sgd}\\
	2\lambda\bRi &= \phantom{\eta \bGi+\eta }  \bNi. \label{eq:RGN_sde}
\end{align}
Combining \eqref{eq:RGN_sgd}, \eqref{eq:RGN_sde}, and \eqref{eq:C_close}, we have 
% \[\eta \frac{\Gi}{\Ni}+1  = \frac{\bNi}{\Ni}\frac{\Ri}{\bRi}(1-\frac{\eta\lambda}{2})\le C^2.\]
\[\eta\Gi + \eta\Ni \le 2\lambda \Ri \le 2\lambda C\bRi= C\bNi.\]
Applying \eqref{eq:C_close} again, we have 
\( \eta\bGi+ \bNi \le C\eta(\Gi + \Ni) \le  C^2\bNi \le C^3\eta \Ni.\)
\end{proof}
\begin{remark}
\Cref{thm:eq_sde_sgd} can be understood from two perspectives. From the viewpoint of approximating a fixed SDE by SGD, it says whenever $\eta > \frac{\bNi}{\bGi}(C^2-1)$, regardless of the shape (i.e., the third-and-higher moments) of the noise, the equilibrium of SGD~\eqref{eq:sgd_wd} won't be $C$-close to the equilibrium of SDE~$\eqref{eq:sde_wd}$. While from the viewpoint of approximating SGD by SDE, it says that the NSR must be at least as large as constant $\frac{1}{C^2-1}$.
\end{remark}
In particular, the order-1 approximation~\eqref{eq:sde_wd} misses a second order term in SGD, $\eta\Gi$. This gap can also be found between \eqref{eq:sde_wd} and other continuous dynamics that are order-2 weak approximations for SGD, e.g., \Cref{eq:2nd_sde} in \citep{li2019stochastic}. 
In \Cref{appsec:omit_proofs_lsr}, we show the equilibrium of order-2 SDE approximation~\eqref{eq:2nd_sde} cannot be $C$-close to that of 1st order SDE approximation~\eqref{eq:motivating_sde} for large LR.

\begin{theorem}[Theorem 9 in \cite{li2019stochastic}]
\eqref{eq:2nd_sde} is an order-2 weak approximation of SGD~\eqref{eq:sgd_iter}:
\begin{equation}\label{eq:2nd_sde}
\begin{split}
	\dd X_t =  -\eta \nabla\big(\Loss(X_t) + \dfrac{\eta}{4}\|\nabla\Loss(X_t)\|_2^2\big) \dd t 
	 + \sqrt{\eta}(\Sigma(X_t))^{1/2}\dd W_t
	\end{split}
\end{equation}
\end{theorem}




%%%% zhiyuan: the curvature regime discussion is not very import
%We can also use $\eta \ge \frac{\Ni}{\Gi}(C^2-1)$ as a more formal definition for the curvature dominated regime proposed in \citep{smith2020generalization} for normalized networks. 
%The original definition in \cite{smith2020generalization} of the critical LR $\eps_{crit}:=2/\lambda_{max}$ is somewhat circular: to know whether a single run with LR $\eta$ belongs to the curvature dominated regime (i.e.,  if $\eta$ is  larger than $\eps_{crit}$), one must first evaluate the $\lambda_{max}$, the largest eigenvalue of the Hessian of the local convex approximation of the loss. Hence, $\lambda_{max}$ depends on the trajectory of SGD, and thus the LR $\eta$ itself! 
%As pointed out by \citep{cohen2021gradient}, the smoothness along the trajectory depends heavily on the chosen LR.
%Compared to the original definition, the new threshold $\frac{\Ni}{\Gi}(C^2-1)$ is well-defined and provides the desired guarantee that LSR induced by successful SDE approximation will break when LR exceeds this threshold.

%Still, there are two pitfalls: first, $\frac{\Ni}{\Gi}$ cannot be measured as simulating the SDE with high precision is computationally expensive; second, in practice, people are often more interested in how closely the performance of large batch SGD matches that of its small batch counterpart, instead of how closely it matches the SDE limit. 
%We address these issues below by adapting the analysis above to understand LSR.


\subsection{Provable Failure of Linear Scaling Rule}
In this section we derive a similar necessary condition for LSR to hold. 
Ideally, we should measure the similarity in terms of train/test loss or accuracy, but the optimization and generalization for deep nets beyond NTK regime~\cite{jacot2018ntk,allenzhu2018convergence,du2018gradient,zou2020gradient,arora2019fine,allenzhu2019learning} is in general still an open problem.
As previous, we will use $\Ri^{B,\eta},\Gi^{B,\eta},\Ni^{B,\eta}$ to denote the limiting squared norm, gradient norm and trace of covariance for SGD~\eqref{eq:sgd_wd} with LR $\eta$ and $\Loss_{\gamma_k}$ a independently sampled random loss with mini-batch of size  $B$.  We first introduce the concept of Linear Scaling Invariance (LSI). Note here we care about the scaled ratio $\Ni^{B,\eta}/(\kappa \Ni^{\kappa B,\kappa\eta})$ because  corvariance scales inversely to batch size, $\Sigma^B(x) = \kappa \Sigma^{\kappa B}(x)$.
\begin{definition}[$(C,\kappa)$-Linear Scaling Invariance]\label{def:lsi}
	We say  SGD~\eqref{eq:sgd_wd} with batch size $B$ and LR $\eta$ exhibits $(C,\kappa)$-LSI if, for a constant $C$ such that $0 < C < \sqrt{\kappa}$,  \vspace{-0.2cm}
\begin{equation}\label{eq:C_kappa_close}
    \frac{1}{C}\le \frac{\Ri^{B,\eta}}{\Ri^{\kappa B,\kappa \eta}},\frac{\Ni^{B,\eta}}{\kappa\Ni^{\kappa B,\kappa\eta}},\frac{\Gi^{B,\eta}}{\Gi^{\kappa B,\kappa \eta}}\le C.
\end{equation}
\end{definition}
%The following results showed that we know if $\frac{\Gi^{\kappa B}}{\Ni^{\kappa B}}$ is larger than constant, then $(C,\kappa)$-LSI fails, even without knowing the baseline value, $\frac{\Gi^B}{\Ni^B}$ 
\vspace{-0.3cm}We show below that $(C,\kappa)$-LSI fails if $\frac{\Gi^{\kappa B,\kappa\eta}}{\Ni^{\kappa B,\kappa\eta}}$ is larger than some setting-dependent constant.
\begin{theorem}\label{thm:lsr_condition}
Assuming $(C,\kappa)$-LSI,  regardless of the value of $\Ri^{B,\eta},\Gi^{B,\eta},\Ni^{B,\eta}$, it holds that

\begin{equation}\label{eq:R_to_GN}
	\frac{\Ni^{\kappa B,\kappa\eta}}{\Gi^{\kappa B,\kappa\eta}}\ge (1-\frac{1}{\kappa})\frac{1}{C^2-1} -\frac{1}{\kappa}
\end{equation}
\end{theorem}

% This theorem gives us a necessary condition for $(C, \kappa)$-LSI without knowing the baseline $\frac{\Gi^B}{\Ni^B}$, but we can also refine the upper bound of $\kappa$ when we have access to the baseline ratio:
In other words, this theorem gives us a certificate for failure of $(C, \kappa)$-LSI without even running the baseline. Interestingly, the following theorem shows we can also predict the largest batch size for which $(C,\kappa)$-LSI holds just with a single run of baseline:

\begin{theorem}\label{thm:lsr_kappa_bound}
Assuming  $(C,\kappa)$-LSI holds, we have\vspace{-0.6cm}

	\[\quad \kappa \le C^2(1+\frac{\Ni^{B,\eta}}{\Gi^{B,\eta}}),\ \ (\approx C^2\frac{\Ni^{B,\eta}}{\Gi^{B,\eta}}\text{ when } \frac{\Ni^{B,\eta}}{\Gi^{B,\eta}}\gg 1).\]
\end{theorem} 

%
%\input{lsi}

%As aforementioned, LSI holds for SDE in~\Cref{eq:motivating_sde}, and therefore for SGD which could be well approximated by SDE. In other words, LSI is a necessary condition for the SDE approximation. In this section, we will show the first failure mode also leads to the failure of LSI in deep learning.
%
%We consider the following dynamics $\{x_k^{\kappa B,\kappa\eta}\}_{k=1}^{\frac{T}{\kappa\eta}}$ under LSR which corresponds to the same 1st order SDE approximation. 
%
%\subsection{A necessary condition for Linear Scale Invariance}
%\input{lsi_analysis}

%\zhiyuan{New experiments to run: lr = 6.4, batch size = 1024, in this ladder, is $G/N$ still a good predictor for the failure of LSI?}
%\zhiyuan{Three outcomes, each is interesting.}
\input{lsi_experiments}
